Sub-Millimeter Variability in the Envelope & Warped Protostellar Disk of the Class 0 Protostar HOPS 358

The JCMT Transient Survey recently discovered that the Class 0 protostar HOPS 358 decreased in 350 GHz continuum brightness by $\sim25$% over the course of four years before brightening again for the next four. The JCMT lightcurve can be fit by a long timescale dip lasting roughly eight years. A shorter timescale periodicity is also apparent with a period of 1.75 years and a small 3% amplitude. NEOWise monitoring reveals that the mid-IR wavelength brightness of HOPS 358 follows a similar long-term pattern in time. Here, we present a study of nine epochs of ALMA observations of HOPS 358 taken over the course of the decline and subsequent rise in brightness seen with the JCMT to test whether the variation seen on $\sim15"$ scales, covering both disk and envelope, is also observed on smaller, $<1"$ scales that primarily probe HOPS 358's protostellar disk. We detect both HOPS 358 and its southern companion, HOPS 358B, in our ALMA observations, and find that at least one of the two is varying. Assuming that HOPS 358 is the variable, the light curve has the same shape as that found by the JCMT. Additionally, our high resolution ALMA imaging of HOPS 358 reveals that the disk is warped, with a $16^{\circ}$ warp at a disk radius of 35 au, about halfway through the extent of the disk. The physical origin of the warp along with how it relates to the variability seen towards HOPS 358, however, remain unclear.

==> baselines_figureset.tex <==
\figsetstart
\figsetnum{5}
\figsettitle{Baseline Matching}

\figsetgrpstart
\figsetgrpnum{figurenumber.1}
\figsetgrptitle{Epoch 3 vs. Epoch 0}
\figsetplot{epoch3_vs_epoch0_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.2}
\figsetgrptitle{Epoch 3 vs. Epoch 1}
\figsetplot{epoch3_vs_epoch1_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.3}
\figsetgrptitle{Epoch 3 vs. Epoch 2}
\figsetplot{epoch3_vs_epoch2_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.4}
\figsetgrptitle{Epoch 3 vs. Epoch 4}
\figsetplot{epoch3_vs_epoch4_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.5}
\figsetgrptitle{Epoch 3 vs. Epoch 5}
\figsetplot{epoch3_vs_epoch5_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.6}
\figsetgrptitle{Epoch 3 vs. Epoch 6}
\figsetplot{epoch3_vs_epoch6_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.7}
\figsetgrptitle{Epoch 3 vs. Epoch 7}
\figsetplot{epoch3_vs_epoch7_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.8}
\figsetgrptitle{Epoch 3 vs. Epoch 8}
\figsetplot{epoch3_vs_epoch8_baselines.pdf}
\figsetgrpnote{Demonstration of the process of matching baselines between two epochs of observations. On the left we show the histograms of $d_{close}$ calculated for each epoch. In the center we show KDE estimates of the distribution of baselines for each epoch of data after the cut of $d_{close} < 0.1$, along with an addition distribution showing the baselines for the epoch matched to Epoch 3. Finally, on the right we show the final, two-dimensional distribution of baselines for the two epochs after this matching routine. We also show all of the trimmed points as faint transparent gray points in the background.}
\figsetgrpend

\figsetend

==> images_figureset.tex <==
\figsetstart
\figsetnum{6}
\figsettitle{Matched Resolution Imaging of HOPS-358}

\figsetgrpstart
\figsetgrpnum{figurenumber.1}
\figsetgrptitle{Epoch 3 vs. Epoch 0}
\figsetplot{epoch3_vs_epoch0_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.2}
\figsetgrptitle{Epoch 3 vs. Epoch 1}
\figsetplot{epoch3_vs_epoch1_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.3}
\figsetgrptitle{Epoch 3 vs. Epoch 2}
\figsetplot{epoch3_vs_epoch2_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.4}
\figsetgrptitle{Epoch 3 vs. Epoch 4}
\figsetplot{epoch3_vs_epoch4_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.5}
\figsetgrptitle{Epoch 3 vs. Epoch 5}
\figsetplot{epoch3_vs_epoch5_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.6}
\figsetgrptitle{Epoch 3 vs. Epoch 6}
\figsetplot{epoch3_vs_epoch6_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.7}
\figsetgrptitle{Epoch 3 vs. Epoch 7}
\figsetplot{epoch3_vs_epoch7_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{figurenumber.8}
\figsetgrptitle{Epoch 3 vs. Epoch 8}
\figsetplot{epoch3_vs_epoch8_images.pdf}
\figsetgrpnote{Comparison of HOPS 358 ({\it top}) and HOPS 358B ({\it bottom}) for each epoch of data with our reference epoch, Epoch 3, when imaged using only baselines matched to Epoch 3 as described in Section \ref{section:alma-flux-comparison}. Though we show the images as well as the difference image between them here for a visual demonstration, our quantitative comparison of the flux between epochs is done by fitting a two-dimensional Gaussian function in the visibility plane to each of the matched datasets. We also note that we have not attempted to correct for uncertainties in the relative flux scaling between epochs, so the peak fluxes and structures in the residuals should be treated with caution. Relative changes between HOPS-358 and HOPS-358B are, however, more reliable.}
\figsetgrpend

\figsetend
